Filter Pruning via Geometric Median for Deep Convolutional Neural Networks Acceleration

Previous works utilized ''smaller-norm-less-important'' criterion to prune filters with smaller norm values in a convolutional neural network. In this paper, we analyze this norm-based criterion and point out that its effectiveness depends on two requirements that are not always met: (1) the norm deviation of the filters should be large; (2) the minimum norm of the filters should be small. To solve this problem, we propose a novel filter pruning method, namely Filter Pruning via Geometric Median (FPGM), to compress the model regardless of those two requirements. Unlike previous methods, FPGM compresses CNN models by pruning filters with redundancy, rather than those with ''relatively less'' importance. When applied to two image classification benchmarks, our method validates its usefulness and strengths. Notably, on CIFAR-10, FPGM reduces more than 52% FLOPs on ResNet-110 with even 2.69% relative accuracy improvement. Moreover, on ILSVRC-2012, FPGM reduces more than 42% FLOPs on ResNet-101 without top-5 accuracy drop, which has advanced the state-of-the-art. Code is publicly available on GitHub: https://github.com/he-y/filter-pruning-geometric-median

==> table/table3_cifar10_nocite.tex <==

%-------------------------------------------------------

%\setlength{\tabcolsep}{1.2mm}
\begin{table*}[th]\small
\centering  	
\begin{tabular}{|c|c c c c c c c|}  		
\hline 		
Depth & Method &Fine-tune? &Baseline acc. (\%)  &Accelerated acc. (\%)  &Acc. $\downarrow$ (\%) & FLOPs & FLOPs $\downarrow$(\%)       
\\ \hline \hline   
\multirow{4}{*}{20}        
%&MIL~\cite{Dong_2017_CVPR} &\xmark        & 91.53        & \textbf{91.43} &0.10 &	3.20E7	  & 20.3	 \\          
& SFP  & \xmark       & \textbf{92.20} ($\pm$0.18)       &  90.83  ($\pm$0.31)& 1.37&  {2.43E7} &{42.2}  \\
& Ours (FPGM-only 30\%) & \xmark       & \textbf{92.20} ($\pm$0.18)       &  {91.09} ($\pm$0.10) & {1.11}&  {2.43E7} &{42.2}  \\  
& Ours (FPGM-only 40\%) & \xmark       & \textbf{92.20} ($\pm$0.18)       &  {90.44} ($\pm$0.20) & {1.76}&  \textbf{1.87E7} &\textbf{54.0}  \\  
& Ours (FPGM-mix 40\%) & \xmark       & \textbf{92.20} ($\pm$0.18)       &  \textbf{91.99} ($\pm$0.15) & \textbf{0.21}&  \textbf{1.87E7} &\textbf{54.0}  \\  

\hline     \hline         

\multirow{5}{*}{32} &MIL  &\xmark       &92.33         & 90.74 &1.59 &	4.70E7	  & 31.2	 \\          
&SFP  & \xmark    & \textbf{92.63} ($\pm$0.70)       &  92.08 ($\pm$0.08)& 0.55 &  {4.03E7} &{41.5} \\ 
& Ours (FPGM-only 30\%)   & \xmark    & \textbf{92.63} ($\pm$0.70)       &  {92.31} ($\pm$0.30) & {0.32} &  {4.03E7} &{41.5} \\   
& Ours (FPGM-only 40\%)   & \xmark    & \textbf{92.63} ($\pm$0.70)       &  91.93 ($\pm$0.03)& 0.70 &  \textbf{3.23E7} &\textbf{53.2} \\
& Ours (FPGM-mix 40\%)   & \xmark    & \textbf{92.63} ($\pm$0.70)       &  \textbf{92.82} ($\pm$0.03) & \textbf{-0.19}&  \textbf{3.23E7} &\textbf{53.2} \\

\hline  \hline   


\multirow{9}{*}{56} 		
&PFEC  &\xmark      & 93.04                   & 91.31  &1.75 &9.09E7  &27.6		 \\         
&CP  &\xmark       & 92.80                      & 90.90 &1.90 &	\textbf{--}	  & 50.0	 \\         

&  SFP  &\xmark  	&\textbf{93.59} ($\pm$0.58)  & 92.26  ($\pm$0.31)& 1.33   &  \textbf{5.94E7} &\textbf{52.6} \\       
& Ours (FPGM-only 40\%)    &\xmark  	&\textbf{93.59} ($\pm$0.58)  & \textbf{92.93} ($\pm$0.49) & \textbf{0.66}   &  \textbf{5.94E7} &\textbf{52.6} \\   
& Ours (FPGM-mix 40\%)    &\xmark  	&\textbf{93.59} ($\pm$0.58)  & {92.89} ($\pm$0.32) & {0.70}   &  \textbf{5.94E7} &\textbf{52.6} \\   

\cdashline{2-8} 

&PFEC  &\cmark      & 93.04          & 93.06 &-0.02 &9.09E7 & 27.6 \\	

&CP  &\cmark        & 92.80                   & 91.80 &1.00 &	\textbf{--}	 &	50.0 	 \\         


& Ours (FPGM-only 40\%)   &\cmark  	&\textbf{93.59} ($\pm$0.58)   &\textbf{93.49} ($\pm$0.13) &\textbf{0.10}   & \textbf{5.94E7} &\textbf{52.6} \\      
& Ours (FPGM-mix 40\%)   &\cmark  	&\textbf{93.59} ($\pm$0.58)   &{93.26} ($\pm$0.03) &{0.33}   & \textbf{5.94E7} &\textbf{52.6} \\ 

\hline    \hline   

\multirow{8}{*}{110}   
&MIL  &\xmark        & 93.63         & {93.44} &{0.19} &	-	  & 34.2 	 \\          
&PFEC  &\xmark   &93.53     & 92.94      &  0.61              & 1.55E8 	&38.6 	 \\          
& SFP   &\xmark  & \textbf{93.68} ($\pm$0.32) 	& 93.38  ($\pm$0.30)& 0.30& {1.50E8} &{40.8}   \\  		
& Ours (FPGM-only 40\%)   &\xmark  & \textbf{93.68} ($\pm$0.32) 	& 93.73  ($\pm$0.23)& -0.05& \textbf{1.21E8} &\textbf{52.3}\\ 
& Ours (FPGM-mix 40\%)   &\xmark  & \textbf{93.68} ($\pm$0.32) 	& \textbf{93.85} ($\pm$0.11) & \textbf{-0.17} & \textbf{1.21E8} &\textbf{52.3}\\ 

\cdashline{2-8} 

&PFEC  &\cmark     & 93.53    & 93.30  &{0.20} 	&1.55E8 	&38.6\\ 
&NISP  &\cmark        & \textbf{--}                   & \textbf{--} &0.18 &	\textbf{--}	 &	43.8 	 \\         

& Ours (FPGM-only 40\%)  &\cmark  & \textbf{93.68} ($\pm$0.32) 	& \textbf{93.74} ($\pm$0.10) &\textbf{-0.16}& \textbf{1.21E8} &\textbf{52.3}   \\  		

\hline  	
\end{tabular}  	
\caption{Comparison of pruned ResNet on CIFAR-10.
In ``Fine-tune?'' column, ``\cmark'' and ``\xmark'' indicates whether to use the pre-trained model as initialization or not, respectively.
The ``Acc.~$\downarrow$'' is the accuracy drop between pruned model and the baseline model, the smaller, the better.
} 	
\label{table:cifar10_accuracy} 
\end{table*}  

%-------------------------------------------------------


==> table/table4_imagenet_nocite.tex <==

\setlength{\tabcolsep}{0.30em} 
\begin{table*}[ht] \small 
\centering 	
\begin{tabular}{|c |c c c c c c c c c|} 		
\hline    		
\multirow{3}{*}{Depth}	   & \multirow{3}{*}{Method}  &\multirow{3}{*}{\shortstack {Fine-\\tune?}}  &\multirow{3}{*}{\shortstack {Baseline\\top-1\\acc.(\%)} }  &\multirow{2}{*}{\shortstack {Accelerated\\top-1\\acc.(\%)} } &\multirow{2}{*}{\shortstack{Baseline\\top-5\\acc.(\%)} }   &\multirow{2}{*}{\shortstack {Accelerated\\top-5\\acc.(\%)} }   &\multirow{3}{*}{\shortstack {Top-1 \\acc. $\downarrow$(\%)} }  &\multirow{3}{*}{\shortstack {Top-5\\acc. $\downarrow$(\%)} } & \multirow{3}{*}{\shortstack {FLOPs$\downarrow$(\%)}}    \\
& & & & & & & & & \\
& & & & & & & & & \\
 \hline     \hline     
            
\multirow{6}{*}{18} &MIL &\xmark   &69.98 &66.33 & 89.24     & 86.94	&3.65	 &2.30   & 34.6		 \\	       		  
%& Ours(30\%) &N &\textbf{70.23$\pm$0.06}	&\textbf{67.25$\pm$0.13} & \textbf{89.51$\pm$0.10}  & \textbf{87.76$\pm$0.06}   &\textbf{2.98}   & \textbf{1.75} & \textbf{41.8} \\\hline       
&SFP~  &\xmark &\textbf{70.28}	&{67.10} & \textbf{89.63}  & {87.78}   &{3.18}   & {1.85} & \textbf{41.8} \\

& Ours (FPGM-only 30\%) &\xmark &\textbf{70.28}	&{67.78} & \textbf{89.63}  & {88.01}   &{2.50}   & {1.62} & \textbf{41.8} \\

& Ours (FPGM-mix 30\%) &\xmark &\textbf{70.28}	&\textbf{67.81} & \textbf{89.63}  & \textbf{88.11}   &\textbf{2.47}   & \textbf{1.52} & \textbf{41.8} \\ \cdashline{2-10}
&Ours (FPGM-only 30\%) &\cmark &\textbf{70.28}	&{68.34} & \textbf{89.63}  & \textbf{88.53}   &{1.94}   & \textbf{1.10} & \textbf{41.8} \\

&Ours (FPGM-mix 30\%) &\cmark &\textbf{70.28}	&\textbf{68.41} & \textbf{89.63}  & {88.48}   &\textbf{1.87}   & {1.15} & \textbf{41.8} \\

  
 \hline     \hline     
 


\multirow{6}{*}{34}	          
%&~\cite{Dong_2017_CVPR} &N   & 73.42          &\textbf{72.99} 	&91.36	 &\textbf{91.19}	&\textbf{0.43} 	&\textbf{0.17} 	& 24.8	\\  

&SFP~ 	&\xmark 	&\textbf{73.92}		&71.83	&\textbf{91.62}   & 90.33   & 2.09  & 1.29 & \textbf{41.1}    \\    
 
 &  Ours (FPGM-only 30\%)	&\xmark	&\textbf{73.92}		&71.79	&\textbf{91.62}   &\textbf{90.70}   & {2.13}  &\textbf{0.92}   & \textbf{41.1}    \\     
   &  Ours (FPGM-mix 30\%)	&\xmark	&\textbf{73.92}		& \textbf{72.11}	&\textbf{91.62}   & {90.69}  &\textbf{1.81}    &{0.93}    & \textbf{41.1}    \\ 
% &  \BB{Ours -new-pure-dist(40\%)}	&\xmark 	&\textbf{73.92}		&70.78	&\textbf{91.62}   & 89.96   & {3.14}  &{1.66}   & \textbf{52.7}    \\     

   \cdashline{2-10} 

 &PFEC~  &\cmark    & {73.23}          & 72.17 	&\textbf{--}	 &\textbf{--} &\textbf{1.06} 	&\textbf{--} 	& 24.2	 \\ 

 &  Ours (FPGM-only 30\%)	&\cmark &\textbf{73.92}		& {72.54}	&\textbf{91.62}   & \textbf{91.13}  & {1.38}   &\textbf{0.49}   & \textbf{41.1}    \\    
 
 & Ours (FPGM-mix 30\%)	&\cmark 	&\textbf{73.92}		&\textbf{72.63}	&\textbf{91.62}   & {91.08}  &{1.29}    & {0.54}  & \textbf{41.1}    \\    
% &  \BB{Ours -new-pure-dist(40\%)}	&\cmark 	&\textbf{73.92}		&71.59	&\textbf{91.62}   & 90.49   & {2.33}  &{1.13}   & \textbf{52.7}     \\     
 \hline      \hline     



\multirow{11}{*}{50}	
&SFP  & \xmark &\textbf{76.15}		&{74.61}		&\textbf{92.87}	  & {92.06} &1.54	 & 0.81 & 41.8  	 \\
& Ours (FPGM-only 30\%) & \xmark  &\textbf{76.15}		&\textbf{75.03}		&\textbf{92.87}	  & \textbf{92.40} &\textbf{1.12} 	 &\textbf{0.47}   &  42.2  	 \\
&  Ours (FPGM-mix 30\%)  & \xmark  &\textbf{76.15}		&{74.94}		&\textbf{92.87}	  & {92.39} &{1.21} 	 & {0.48}  & 42.2  	 \\
&   Ours (FPGM-only 40\%) & \xmark  &\textbf{76.15}		&{74.13}		&\textbf{92.87}	  & {91.94} & {2.02}	 &{0.93}  & \textbf{53.5}  	 \\


\cdashline{2-10} 
&ThiNet   &\cmark  &72.88 	&72.04  & 91.14   & 90.67              & {0.84} 	&{0.47}	& 36.7  \\  		  
&SFP~  & \cmark  &\textbf{76.15}		&{62.14}		&\textbf{92.87}	  & {84.60} &14.01	 & 8.27 & 41.8  	 \\
&NISP~ & \cmark  &\textbf{--}		&\textbf{--}	&\textbf{--}	  & \textbf{--} & 0.89	 & \textbf{--}& 44.0  	 \\
&CP  &\cmark 	&\textbf{--}	&\textbf{--} & 92.20    &90.80  	&\textbf{--}	& 1.40	 &{50.0}	 	\\     		  

&   Ours (FPGM-only 30\%)  & \cmark  &\textbf{76.15}		&\textbf{75.59}		&\textbf{92.87}	  & \textbf{92.63} & \textbf{0.56}	 &{0.24}  & 42.2  	 \\

&  Ours (FPGM-mix 30\%)       &\cmark &\textbf{76.15}		&{75.50}		&\textbf{92.87}	  & {92.63} &{0.65} 	 &\textbf{0.21}  & 42.2  	 \\
&  Ours (FPGM-only 40\%)  & \cmark  &\textbf{76.15}		&{74.83}		&\textbf{92.87}	  & {92.32} & {1.32}	 &{0.55}  &\textbf{53.5}   	 \\

\hline   \hline     


\multirow{2}{*}{101}

%& Ours (30\%) & \xmark  &\textbf{77.37}		& 77.03 	&\textbf{93.56}	  &  93.46  & 0.34 	 &  0.10  & {42.2}    \\ 
%\cdashline{2-10}ijump2(){}

& Rethinking~  & \cmark  &\textbf{77.37}		& 75.27 	&\textbf{--}  &  \textbf{--}  & 2.10 	 &  \textbf{--}  & \textbf{47.0}    \\  
& Ours (FPGM-only 30\%) &\cmark  &\textbf{77.37}		&\textbf{77.32}		&\textbf{93.56}	  & \textbf{93.56} &\textbf{0.05}	 & \textbf{0.00}& {42.2}    \\ 		
\hline    	
\end{tabular} 	
\caption{
Comparison of pruned ResNet on ILSVRC-2012.
``Fine-tune?'' and "acc. $\downarrow$" have the same meaning with Table~\ref{table:cifar10_accuracy}.
%We run ResNet-18 for three times to get the mean and std.
%For the other depths of ResNet, we just list the one-view accuracy.
} 
\label{table:imagenet_accuracy}
\end{table*}

